Regular Separability in B\"{u}chi VASS

We study the ($\omega$-)regular separability problem for B\"uchi VASS languages: Given two B\"uchi VASS with languages $L_1$ and $L_2$, check whether there is a regular language that fully contains $L_1$ while remaining disjoint from $L_2$. We show that the problem is decidable in general and PSPACE-complete in the 1-dimensional case, assuming succinct counter updates. The results rely on several arguments. We characterize the set of all regular languages disjoint from $L_2$. Based on this, we derive a (sound and complete) notion of inseparability witnesses, non-regular subsets of $L_1$. Finally, we show how to symbolically represent inseparability witnesses and how to check their existence.

==> regsep-vs-intersection.tex <==
We present a class of WSTS such that, for their $\omega$-languages, intersection is decidable whereas regular separability is
not. 
%
%
%
A $d$-dimensional \emph{reset B\"{u}chi VASS} over alphabet $\Sigma$ is a tuple $\cV=(Q,q_0,T,F)$. 
The only difference to B\"uchi VASS is in the finite set of transitions which, besides adding a vector, may reset a counter,  $T\subseteq
Q\times(\Z^d\cup \{\reset_1,\ldots,\reset_d\})\times\Sigma^*\times Q$. 
%
The configurations are defined like for B\"uchi VASS, but the transition relation has to be adapted.  
We have $(q,\bmm) \xrightarrow{w} (q',\bmm')$ if there is a transition
$(q,x,w,q')$ such that either
\begin{myenum}
\myitem $x\in\Z^d$ and $\bmm'=\bmm+x$ or
\myitem $x=\reset_i$ for some $i\in[1,d]$ and $\bmm'(j)=\bmm(j)$ for $j\in[1,d]\setminus\{i\}$ and $\bmm'(i)=0$.
\end{myenum}
Acceptance is defined as before, and so is the language (of infinite words) $L(\cV)$. 
\begin{comment}
In other words, a transition in $Q\times\Z^d\times\Sigma^*\times Q$ induces the
same steps as in an ordinary VASS. But a transition of the form
$(q,\reset_i,w,q')$ resets the $i$-th counter to zero. Such transitions are
called \emph{reset transitions}. The language of $\cV$ is then defined as
\[ L(\cV) =\{w_1w_2\cdots\in\Sigma^\omega \mid \text{$\exists$~a run $(q_0,\bzero)\xrightarrow{w_1}(q_1,\bmm_1)\xrightarrow{w_2}\cdots$ that visits $F$ infinitely often} \}. \]
\end{comment}

For general B\"{u}chi reset VASS, emptiness and intersection are undecidable~\cite[Theorem~10]{Mayr2003}. 
We consider a slight restriction of the model that makes the problems decidable.
%
A B\"{u}chi reset VASS is \emph{weak} if there is no path from a final state to a reset transition. In particular, an
accepting run can only perform finitely many resets. Note that the usual
product construction of $\cV_1$ and $\cV_2$ to yield a B\"{u}chi reset VASS
for $L(\cV_1)\cap L(\cV_2)$ preserves weakness. 
\begin{theorem}
For weak B\"{u}chi reset VASS, emptiness (hence intersection) is decidable.
\end{theorem}
Here, emptiness can be decided using standard techniques. We order the
configurations $Q\times\N^d$ in the usual way: We have $(q,\bmm)\le (q',\bmm')$
if $q=q'$ and $\bmm\le\bmm'$. First, one observes that for any
B\"{u}chi VASS $\cV$, the set $U(\cV)\subseteq Q\times\N^d$ of all
configurations $(q,\bmm)$ from which an infinite accepting run can start, is
upward closed. Moreover, using a saturation procedure, we can effectively
compute the finitely many minimal elements
$(q_1,\bmm_1),\ldots,(q_\ell,\bmm_\ell)$ of $U(\cV)$. The details are in the appendix.
Then, for a weak
B\"{u}chi reset VASS $\cV$, we do the following. We construct the B\"{u}chi
VASS $\cV'$, which is obtained from $\cV$ by deleting all reset transitions.
Now $L(\cV)$ is non-empty if and only if $\cV$, as a reset VASS, can cover any
of the configurations $(q_1,\bmm_1),\ldots,(q_\ell,\bmm_\ell)$ of $U(\cV')$.
Whether the latter is the case can be decided because coverability is decidable
in reset
VASS~\cite{DBLP:conf/icalp/DufourdFS98,DBLP:journals/tcs/FinkelS01,DBLP:journals/iandc/AbdullaCJT00}.

\begin{theorem}\label{regsep-undecidable-wbrvass}
For weak B. reset VASS over $\Sigma_1$, regular separability from $D_1$ is undecidable.
\end{theorem}
We reduce from the place boundedness problem for reset VASS.
%
A reset VASS is a B\"{u}chi reset VASS without input
words and without final states. 
%
For $k\in\N$, we say that a reset VASS $\cV$ is \emph{$k$-place bounded}
if for every reachable configurations $(q,\bmm)$, we have $\bmm(1)\le k$. 
%
Moreover, we call $\cV$ \emph{place bounded} if $\cV$ is $k$-place bounded for some $k\in\N$.
%
The \emph{place boundedness problem} then asks whether a given reset VASS is place bounded.
%
%
%
%
The place boundedness problem (more generally, the boundedness problem) for
reset VASS is known to be undecidablei~\cite[Theorem
8]{DBLP:conf/icalp/DufourdFS98} (for a simpler proof, see \cite[Theorem
18]{Mayr2003}).
%
%
%
%
%

\input{weak-buechi-reset-vass}
%
%
%
%
%
Given a $d$-dim.\ reset VASS $\cV$, we build a $(d+1)$-dim.\ weak B\"{u}chi reset VASS $\cV'$ with
        \begin{align}
		L(\cV')=\{ w\in S_{1,k} \mid k\in\N,~\text{$\cV$ can reach some $(q,\mathbf{m})\in Q\times\N^d$ with $\bmm(1)\ge k$}\}.\label{weak-buechi-reset-vass-language}
        \end{align}
	Before we describe $\cV'$, observe that $\regsep{L(\cV')}{D_1}$ iff
	$\cV$ is place bounded. If $\cV$ is $k$-place bounded, then
	$L(\cV')\subseteq S_{1,k}$ and thus $\regsep{L(\cV')}{D_1}$. On the
	other hand, if $\cV$ is not place bounded, then
	$L(\cV')=\bigcup_{k\in\N} S_{1,k}$. As for the B\"{u}chi VASS in
	\cref{Figure:examples} (left), one can show $\notregsep{L(\cV')}{D_1}$.

The construction is depicted in \cref{figure:weak-buechi-reset-vass}.  
%
The dashed box contains
	$\cV_\varepsilon$, which is obtained from $\cV$ by changing every
	transition $(p,\bu,q)$ into $(p,(\bu,0),\varepsilon,q)$. In the figure, $q$
	stands for arbitrary states of $\cV_\varepsilon$, meaning for every
	state $q$ in $\cV_\varepsilon$, we have a transition
	$(q,\bzero,\varepsilon,q_1)$.  Observe that in the states
	$q_1,q_2,q_3$, $\cV'$ behaves exactly like the B\"{u}chi VASS in
	\cref{Figure:examples}(left), except that the additional counter
  ensures that for each infix the balance on letter $a_i$ is bounded by $k$
  from configurations $(q_1, (k, \bu))$.
  Thus the accepted language from $(q_1, (k, \bu))$ is exactly $S_{1,k}$.
	This shows that $\cV'$ accepts the language
	\eqref{weak-buechi-reset-vass-language}.



